Edge Computing for User-Centric Secure Search on Cloud-Based Encrypted Big Data

Cloud service providers offer a low-cost and convenient solution to host unstructured data. However, cloud services act as third-party solutions and do not provide control of the data to users. This has raised security and privacy concerns for many organizations (users) with sensitive data to utilize cloud-based solutions. User-side encryption can potentially address these concerns by establishing user-centric cloud services and granting data control to the user. Nonetheless, user-side encryption limits the ability to process (e.g., search) encrypted data on the cloud. Accordingly, in this research, we provide a framework that enables processing (in particular, searching) of encrypted multi-organizational (i.e., multi-source) big data without revealing the data to cloud provider. Our framework leverages locality feature of edge computing to offer a user-centric search ability in a real-time manner. In particular, the edge system intelligently predicts the user's search pattern and prunes the multi-source big data search space to reduce the search time. The pruning system is based on efficient sampling from the clustered big dataset on the cloud. For each cluster, the pruning system dynamically samples appropriate number of terms based on the user's search tendency, so that the cluster is optimally represented. We developed a prototype of a user-centric search system and evaluated it against multiple datasets. Experimental results demonstrate 27% improvement in the pruning quality and search accuracy.

==> Sources/clusterrepo.tex <==
\section{Identify User Search Pattern}\label{sec:userSearchPattern}
To represent an encrypted data set is complex.  The data owner didn't want the data will be decrypted in the cloud.  So, we can't touch the encrypted data. But we can understand what kinds of terms are being searched by the user.  Here we use the basic Markov Chain Model to identify the most popular term which will be searched by the user in near future. 

==> Sources/method-sample.tex <==
\section{Constructing sample of an encrypted cluster}\label{sec:method}
\subsection{Overview}
Recall that there is a one-to-one association between a sample and a cluster. In fact, each sample is a representative of its corresponding cluster that resides on the edge tier, can be quickly compared against the search query, and navigates the search only to relevant clusters (\ie pruning). 

Accurate pruning and choosing the relevant cluster strongly depends on how representative the corresponding sample is. In fact, quantity and quality of sampled terms from a cluster determine representativeness of the sample. The \emph{quantity} refers to the sample size from the corresponding cluster whereas the \emph{quality} of the sample depends on the how the chosen terms conceptually express the cluster. 
As for the optimal sample size, we should note that, too small sample size impacts representativeness of the sample and inaccuracy of pruning that subsequently affects the search precision. On the other hand, too large sample size impacts the real-time feature of the search operation. 

The search precision is impacted by the samples' quality. For a given search query, based on the semantic relatedness between samples and the query, the pruner determines which clusters on the cloud must be excluded or included in the search operation. Therefore, each sampled term should semantically represent a portion (\ie sub-topic) of the corresponding cluster and the union of sampled terms must represent the topics of the entire cluster. Moreover, the sample should reflect the changes occur to the dataset (\ie the changes happen because of document addition or removal). As such, the sample manager should have the flexibility of dropping sampled terms that lose their importance over time and replacing them by more representative ones. 

According to Figure~\ref{fig:systemArchitecture}, the Sample Manager module in edge tier is in charge of constructing and populating samples. As the terms in the clusters are encrypted, the Sample Manager cannot use them to build samples and address the expected demands. Therefore, we propose to construct the samples based on other available metadata. In particular, quality and quantity of the sample terms are determined based on the following factors: \textit{user search pattern}, \textit{variation of interests to a cluster}, and \textit{number of cluster terms} (aka cluster size). In the rest of this section, we elaborate on how to consider these factors on a given cluster to determine terms in its corresponding sample.
%We utilize the above mention factors information to add or replace the in the sample while maintaing the optimal quality of abst
%For adding or replacing an item in the sample, we consider a semantic replacable radius value. To calculate semantic radius value, we use the value returned by the above mention three factors. The qualification of any term to add or replace dynamically in the sample, we use the weight return by the Markov Chain Model for the term.  Through this way, we eventually maintain the optimal number of terms in the sample dynamically with respect to time. 

\subsection{Identify Users' Search Pattern}
%Sampling encrypted terms in clusters without decrypting them is infeasible, as their true meaning (semantic) is lost. To overcome this problem,
Sample Manager considers users' search pattern as an accessible metadata and leverage that for quality sampling that can semantically project the topics of the cluster. %Specifically, by analyzing the metadata, we are able to infer the terms in the clusters and create a sample . 
In addition, analyzing search pattern enables us to learn about search queries that potentially appear in near future. This knowledge can be leveraged to improve the precision of pruning and subsequently the search operation. Recall that search pattern analysis occurs in the edge tier that is considered to be at the user's premises, hence, trustworthy. 

%sample of any cluster data eventually helps to understand the topic of the data which is very helpful while searching data into the cluster. When any search data compare with the sample of cluster data, then it can identify which cluster actually related to the search query based on the topic relativeness.  But to represent an encrypted cluster data isn't possible when the system isn't allowed to decrypt the data while uploading or searching process. Only the user can decrypt data when the final result of search query sends back to the user. So, the system can't decrypt the encrypted data in the cloud but it has to make an appropriate representation of the encrypted cluster data to understand the topic of the cluster. To overcome this problem, we consider the user search pattern as a solution.  The user search pattern widely used to make a system prepare better for the situation based on previous experience. We also used this technique to understand what can be the potential search word on the system and prepare the sample for those search. 

%The search word first comes to the edge server from users and then to the cloud. In the edge, we monitor the search word for corresponding cluster. Thus how we can understand what kinds of terms are being searched by the user in the cluster.  Among the search list, we identify the most popular and generalized search word which is efficient enough to represent cluster data, which we call as an sample. We use the Markov Chain Model to identify the most popular terms which will be searched in near future. We consider those terms as a potential candidate to the sample element.

For the prediction, we develop a method based on Markov Chain model, because it can describe a sequence of possible events where the probability of each event depends only on the state attained in the previous event. For that purpose, we create an adjacency graph that contains the sequence of search queries made by users to a particular cluster and leverage that to predict search queries potentially can appear in the near future. Let $W$ be the set of searched terms appear in the system during certain time period (in form of $W:\{w_1, w_2, ....,w_n\}$) that hit a particular cluster $c$. Elements of this set can be considered as states of Markov Chain. We define \emph{transition probability} from $w_i$ to $w_j$ (denoted $P_{ij}$) as the likelihood that a user searches term $w_j$ after $w_i$. Figure~\ref{fig:userSearchPattern} depicts an example of such transition probabilities on the edges of the graph. The \emph{state probability} for term $w_i$ is defined as the likelihood of the term being searched in future.
Initially, the state probability for $w_i$ is calculated based on the ratio of searching frequency for $w_i$ to the total number of searched terms in cluster $c$. Let the total number of searched terms in cluster $c$ is $n$, then we configure the Markov Chain model for $W$ based on Equation~\ref{eq:markov}. 
%w_{ij} is the transaction probability. The state prob matrix multiply with transaction matrix which produce new state prob matrix.
\begin{equation}\label{eq:markov}
w_{ij}(n)= \sum_{k=1}^{m}w_{ik}(n-1) P_{kj}
\end{equation}

\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{images/userSearchPattern.pdf}
\caption{An overview of user search pattern analysis by using Markov Chain model.
The user search term denotes as the state (rectangle). The arrow and the number shows between arrow represent the transition probability from one state to another. The oval shape denotes the start and end of a session.}
\label{fig:userSearchPattern}
\end{figure}

In the next step, the Markov Chain model predicts each state (term) probability after $n$ steps. We run the model iteratively until the state (term) probability value is converged.  After converging, the model provides us with a weighted list of terms (called \emph{sample candidate}) where the weight represents the probability of a search term appears in near future. We use the term weight to add or replace an item in the sample structure. A term with a higher weight can replace an existing term with a lower weight. 

% We run the model iteratively until the value is converged.  After converging, the model gives us a word list with weight. We sorted out the terms based on weight.  Thus we can know the probability of a search word appear probability in near future. 



\subsection{Variation of Interests to a Cluster}

The number of search queries ($SN$) fall to a cluster can infer us the nature of topics held by the cluster. If a cluster receives more search query compare to another cluster, then that cluster can potentially contains several topics that covers a wider range of search queries. There is also the possibility that the cluster contains topic which is semantically relevant. To capture this, we measure the average semantic similarity distance (denoted as $ASD$) of all search queries that fall into a cluster. If the $ASD$ value is low, it means that the cluster contains data of several topics whereas a higher value means that the cluster is around a topic. Based on the $SN$ on a cluster and its $ASD$ value, we compute the user interest value (denoted $UI$) for a cluster. So, the $UI$ value for $i$th cluster is calculated using Equations~\ref{eq:ASD}, \ref{eq:SN}, and~\ref{eq:UI}.

\begin{equation}\label{eq:ASD}
ASD_i = \frac{ \sum_{k=1}^{n}\sum_{j=1}^{n}SemanticSimilarity(term_{kj})}{n}
\end{equation}

\begin{equation}\label{eq:SN}
SN_i= \frac{SN_i-SN_{avg}}{SN_{avg}}
\end{equation}

\begin{equation}\label{eq:UI}
UI_i = ASD_i + SN_i
\end{equation}

\subsection{Cluster Size}
The cluster size (denoted $CI$) helps to determine the sample size. The sample from large cluster should contains more item compare to the sample formed from small cluster. Therefore, while determining sample size for the cluster, we consider the number of terms in a cluster. First, we determine the average number of terms in the clusters. Then, we calculate the percentage of terms in a cluster with the average number of terms in the cluster. The positive value means the cluster is larger than the average size and a negative value means the cluster is small compared to the average. An sample should have more item for a larger cluster and a small cluster sample should have less item. So the cluster size for $i$th cluster is calculated by Equation~\ref{eq:CI}.

\begin{equation}\label{eq:CI}
CI_i = \frac{ClusterSize_i}{AverageClsuterSize}
\end{equation}


\subsection{Term Addition and Removal in samples}
To create initial sample,  we follow the procedure from S3BD ~\cite{woodworth2018s3bd}. It has fixed 10 terms in the sample and those terms are chosen from the most frequently appear term in the index which has higher associated document list in a cluster. 

We consider semantic radius ($SR$) as the base to add or replace any term in the sample, we calculate the $SR$  for $i$th cluster using Equation~\ref{eq:S42}.
\begin{equation} \label{eq:S42}
SR_i = UI_i + CI_i
\end{equation}

Within the $SR$ range only one term is optimal enough to represent a sub topic. The $SR$ is the base element to add or replace any term to sample.
By analyzing the user search pattern, we have the list of the potential search term with associated weight (\ie Sample Candidate) that may potentially appear in the near future. We calculate the semantic similarity distance between the sample candidate and existing term in the sample. If the calculated semantic distance is lower than the $SR$, it means that there is no existing member in the sample that can represent the sub topic introduced by the search term. Hence, we add that sample candidate to the sample. However, if the calculated semantic distance is higher than the $SR$, then that sample candidate and the member or members of the samples compete for the position in the sample. All of the competing terms' weight are calculated and only the highest weight term will be placed in the sample and others are be discarded.

We explain visually the competition for sample position in Figure~\ref{fig:SR2Image}. In this example, the current sample have only one member, \textit{Viewer}. Now, \textit{Frozen, Wine, Broadway, Mirror, Photo} are the sample candidate. The $SR$ value for the cluster is $0.38$. All the sample candidate check the semantic similarity distance with \textit{Viewer} and compare the value with $SR$. The calculated semantic similarity distance of \textit{Frozen} and \textit{Viewer} is $0.0$. So, \textit{Frozen} represents a different topic that is not covered by the Viewer. So \textit{Frozen} is added to the sample. Now, \textit{Wine, Broadway, Mirror, Photo} semantic similarity distance with \textit{Viewer} is higher than the $SR$ value. So, all those terms along with \textit{Viewer} (the existing sample member) run the competition for the position in sample. Now, the weight calculated from user search pattern for those terms will be checked and only the highest weighted term will be added to sample and others will be discarded.

\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{images/SemanticReplacibleRadius.pdf}
\caption{The sample candidate competing for position in sample based on Semantic Radius. The red colored term is the existing term in the sample. The red dotted circle represents the semantic radius calculated for the cluster. The semantic radius value present by the green color. The blue colored term represents the term present within the semantic radius of the sample term. The black colored term is outside of the semantic radius of the circle. The semantic similarity between the term in the sample and other terms shows in number.}
\label{fig:SR2Image}
\end{figure}

The status of the member of the sample change over time. When any member of sample is not searched by the users or any other semantically related term gain user interest, the old term loses its position in the sample. In this manner, our method ensures the optimal number of terms in the sample and it also make sure that the terms in the sample has a significant contribution to represent a small portion of the cluster or we can say sub topic.%We can think a bunch of little clusters that make the bigger cluster. If we can represent the small cluster, collectively we can represent the whole cluster.


==> Sources/userSearchPattern.tex <==
\section{Identify User Search Pattern}\label{userSearchPattern}
Representation of any cluster data eventually helps to understand the topic of the data which is very helpful while searching data into the cluster. When any search data compare with the representations of cluster data, then it can direct which cluster actually related to the search query based on topic relativeness.  But to represent an encrypted cluster data isn't possible when the system isn't allowed to decrypt the data. So, the system can't touch the encrypted data in the cloud but it has to make an appropriate representation of the cluster to understand the topic of the cluster. To overcome this problem, we consider the user search pattern as a solution. We can understand what kinds of terms are being searched by the user in the cluster. However, to collect all user search isn't needed to make the representation of a cluster.  The most popular and distinct search word is enough for the efficient cluster representation data which we call as an abstract. We use the Markov Chain Model to identify the most popular terms and using word similarity distance for the distinct word which will be searched in near future.  By using the knowledge provided by the Markov Chain Model and word similarity distance we populate the terms in the abstract.
